Peer-to-Peer (P2P) Electricity Markets for Low Voltage Networks

We develop a clearance and settlement model for Peer-to-Peer (P2P) energy trading in low-voltage networks. The model enables direct transactions between parties within an open and distributed system and integrates unused capacity while respecting network constraints. We evaluate the model through simulations of different scenarios (normal operating conditions and extreme conditions) for 24-hour time blocks. Our simulations highlight the benefits of our model in a decentralized energy system, notably its ability to deal with high-trade volumes.

==> data/Makefile <==
#
R=R CMD BATCH

RFILES=p2p_load.R\
       solar_clusters.R\
       residential_clusters.R

OUTFILES=$(RFILES:.R=.Rout)

PDFFILES=../figures/p2p_load.pdf\
	 ../figures/solar_clusters.pdf\
	 ../figures/residential_clusters.pdf

EMBEDFILES=$(PDFFILES:%.pdf=embed_%.pdf)

.PHONY:all clean

#all: $(EMBEDFILES) 
all: $(OUTFILES) 

$(EMBEDFILES): $(PDFFILES)

$(PDFFILES): $(OUTFILES)

embed_%.pdf: %.pdf
	gs -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress -dEmbedAllFonts=true -sOutputFile=$@ -f $<

%.pdf: %.Rout

%.Rout: %.R
	${R} $< >/dev/null

clean:
	rm -f *.pdf *.bak *.Rout


==> data/networks.tex <==
%\documentclass{article}
%\usepackage{tikz}
%\usepackage{pgfplotstable} % for CSV data

%\pgfplotsset{compat=1.18} 
%\begin{document}

%\pgfplotstableread[col sep=comma]{data/pos_edges_list.csv}\nodetable
%\pgfplotstabletypeset{\nodetable}


%\begin{figure}[htbp]
%\centering
%\begin{tikzpicture}[scale=0.01]  

%\pgfplotstableread[col sep=comma]{data/pos_edges_list.csv}\nodetable
%\pgfplotstableread[col sep=comma]{data/edges_list.csv}\edgetable

% Loop through the nodes and create named coordinates 
% Already had ordered pos, but some issue with positioning, this should get a tree like. 
%\pgfplotstableforeachcolumnelement{Node}\of\nodetable\as\nodename{
%    \pgfplotstablegetelem{\pgfplotstablerow}{Y}\of\nodetable
%    \edef\ycoord{\pgfplotsretval}
%    \pgfplotstablegetelem{\pgfplotstablerow}{X}\of\nodetable
%    \edef\xcoord{\pgfplotsretval}
%    \coordinate (\nodename) at (\xcoord,\ycoord);
%}

% Loop through the edges and link nodes
% does not like more than 1 branch... Not going to write recursive funtions in this thing to generate the tree
%\pgfplotstableforeachcolumnelement{Source}\of\edgetable\as\source{
%    \pgfplotstablegetelem{\pgfplotstablerow}{Target}\of\edgetable
%    \edef\target{\pgfplotsretval}
%    \draw[->] (\source) -- (\target);
%}


%\end{tikzpicture}
%\caption{Graph with Edges}
%\end{figure}

%\end{document}


==> tables/tab-extreme-80.tex <==
\begin{table}[ht!]
  \centering
  \caption{Extreme P2P Trades -- 80 bus system}  
  \begin{adjustbox}{width=0.8\columnwidth,center}
    \begin{tabular}{cccc}
      \toprule
        \textbf{Hour} & \textbf{Seller (Bus)} & \textbf{$x_t$} & \textbf{Power (kWh)} \\
      \midrule
      11 & Seller 0 (Bus 11) & 0.853 & 103.707 \\
      11 & Seller 1 (Bus 13) & 0.853 & 103.707 \\
      11 & Seller 2 (Bus 47) & 0.853 & 103.707 \\
      11 & Seller 3 (Bus 45) & 0.853 & 103.707 \\
      11 & Seller 4 (Bus 15) & 0.853 & 103.707 \\
      11 & Seller 5 (Bus 17) & 0.853 & 103.707 \\
      11 & Seller 6 (Bus 19) & 0.853 & 103.707 \\
      11 & Seller 7 (Bus 37) & 0.853 & 103.707 \\
      11 & Seller 8 (Bus 39) & 0.853 & 103.707 \\
      11 & Seller 9 (Bus 41) & 0.853 & 103.707 \\
      11 & Seller 10 (Bus 43) & 0.853 & 103.707 \\
      11 & Seller 11 (Bus 47) & 0.853 & 103.707 \\
      11 & Seller 12 (Bus 77) & 0.853 & 103.707 \\
      11 & Seller 13 (Bus 49) & 0.853 & 103.707 \\
      11 & Seller 14 (Bus 51) & 0.853 & 103.707 \\
      11 & Seller 15 (Bus 58) & 0.853 & 103.707 \\
      11 & Seller 16 (Bus 60) & 0.853 & 103.707 \\
      11 & Seller 17 (Bus 71) & 0.853 & 103.707 \\
      11 & Seller 18 (Bus 73) & 0.853 & 103.707 \\
      11 & Seller 19 (Bus 75) & 0.853 & 103.707 \\
      \midrule
      \multicolumn{2}{c}{\textbf{Total Load}} & \multicolumn{2}{c}{2098.214} \\
      \midrule
      \multicolumn{2}{c}{\textbf{Total P2P Generation}} & \multicolumn{2}{c}{2074.138} \\
      \midrule
      \multicolumn{2}{c}{\textbf{Slack I/E}} & \multicolumn{2}{c}{80.835} \\
      \bottomrule
    \end{tabular}
  \end{adjustbox}
  \label{tab:extreme_80} 
\end{table}



==> tables/tab-percent-res_80.tex <==
\begin{table}[ht!]
\centering
\caption{\% Load Fulfilled w/ P2P -- 80 bus system -- 24 hour Period}
\begin{adjustbox}{width=0.8\columnwidth,center}
\begin{tabular}{ccc}
\toprule
\textbf{Hour} & \textbf{Trade Qt (kWh)} & \textbf{\% Load Fulfilled w/ P2P} \\
\midrule
0--5 & - & - \\
6 & $< 0.01$ & $< 1 \%$ \\
7 & $0.420$ & 0.92 \% \\
8 & $4.640$ & 10.00 \% \\
9 & $15.320$ & 32.99 \% \\
10 & $20.520$ & 43.86 \% \\
11 & $24.300$ & 51.52 \% \\
12 & $24.780$ & 48.84 \% \\
13 & $22.140$ & 38.70 \% \\
14 & $18.160$ & 24.36 \% \\
15 & $12.440$ & 24.62 \% \\
16 & $5.820$ & 10.15 \% \\
17 & $0.020$ & 0.310 \% \\
18--23 & - & - \\
\bottomrule
\end{tabular}%
\end{adjustbox}
\label{tab:results_80_res}
\end{table}


==> tables/tab-percert-res.tex <==
\begin{table}[ht!]
\centering
\caption{\% Load Fulfilled w/ P2P -- 44 bus system -- 24 hour period}
\begin{adjustbox}{width=0.8\columnwidth,center}
\begin{tabular}{ccc}
\toprule
\textbf{Hour} & \textbf{Trade Qt (kWh)} & \textbf{\% Load Fulfilled w/ P2P} \\
\midrule
0--5 & -- & -- \\
6 & $< 0.01$ & $< 1\%$ \\
7 & $0.126$ & 0.928\% \\
8 & $1.392$ & 10.03\% \\
9 & $4.596$ & 32.464\% \\
10 & $6.156$ & 42.923\% \\
11 & $7.290$ & 50.231\% \\
12 & $7.434$ & 52.274\% \\
13 & $6.642$ & 47.685\% \\
14 & $5.448$ & 37.974\% \\
15 & $3.732$ & 24.069\% \\
16 & $1.746$ & 10.098\% \\
17 & $0.060$ & 0.319\% \\
18-23 & -- & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:results_44_res}
\end{table}

==> tables/tab_eco-benefits.tex <==
\begin{table}[ht]
  \caption{Benefit for Buyers and Sellers per Hour Block (80-bus system case)}
  \centering
  \begin{adjustbox}{width=0.9\columnwidth,center}
  \begin{tabular}{cccc}
    \toprule
    \textbf{Hour} & \textbf{Trade Quantity (KWh)} & \textbf{Buyers' Benefit (\$)} & \textbf{Sellers' Benefit  (\$)} \\
    \midrule
    0--5 & - & - & - \\
    6  & $< 0.001$ & $< 0.001$ & $< 0.001$ \\
    7  & 0.420 & 0.063 & 0.021 \\
    8  & 4.640 & 0.696 & 0.232 \\
    9  & 15.320 & 2.298 & 0.766 \\
    10 & 20.520 & 3.078 & 1.026 \\
    11 & 24.300 & 3.645 & 1.215 \\
    12 & 24.780 & 3.717 & 1.239 \\
    13 & 22.140 & 3.321 & 1.107 \\
    14 & 18.160 & 2.724 & 0.908 \\
    15 & 12.440 & 1.866 & 0.622 \\
    16 & 5.820 & 0.873 & 0.291 \\
    17 & 0.020 & 0.003 & 0.001 \\
    18--23 & - & - & - \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \label{tab:eco_benefits}
\end{table}
